Microwave-free vector magnetometry with nitrogen-vacancy centers along a single axis in diamond

Sensing vector magnetic fields is critical to many applications in fundamental physics, bioimaging, and material science. Magnetic-field sensors exploiting nitrogen-vacancy (NV) centers are particularly compelling as they offer high sensitivity and spatial resolution even at nanoscale. Achieving vector magnetometry has, however, often required applying microwaves sequentially or simultaneously, limiting the sensors' applications under cryogenic temperature. Here we propose and demonstrate a microwave-free vector magnetometer that simultaneously measures all Cartesian components of a magnetic field using NV ensembles in diamond. In particular, the present magnetometer leverages the level anticrossing in the triplet ground state at 102.4 mT, allowing the measurement of both longitudinal and transverse fields with a wide bandwidth from zero to megahertz range. Full vector sensing capability is proffered by modulating fields along the preferential NV axis and in the transverse plane and subsequent demodulation of the signal. This sensor exhibits a root mean square noise floor of about 300 pT/Hz^(1/2) in all directions. The present technique is broadly applicable to both ensemble sensors and potentially also single-NV sensors, extending the vector capability to nanoscale measurement under ambient temperatures.

==> supplementary_information.tex <==
%\begin{document}
\begin{comment}
\title{Supplementary Information: Microwave-free vector magnetometry with nitrogen-vacancy centers along a single axis in diamond}% Force line breaks with \\
\author{Huijie Zheng}
\email{zheng@uni-mainz.de}
\affiliation{Johannes Gutenberg-Universit{\"a}t Mainz, 55128 Mainz, Germany}
\author{Zhiyin Sun}
\email{zhiyisun@uni-mainz.de}
%\affiliation{Johannes Gutenberg-Universit{\"a}t Mainz, 55128 Mainz, Germany}
\affiliation{Laboratory for Space Environment and Physical Sciences, Harbin Institute of Technology, 150001 Harbin, China}
\affiliation{Helmholtz Institut Mainz, 55099 Mainz, Germany}
\author{Georgios Chatzidrosos}
\affiliation{Johannes Gutenberg-Universit{\"a}t Mainz, 55128 Mainz, Germany}
\author{Chen Zhang}
\affiliation{Institute of Physics, University of Stuttgart and Institute for Quantum Science and Technology IQST, 70174 Stuttgart, Germany}
\author{Kazuo Nakamura} 
\affiliation{Application Technology Research Institute, Tokyo Gas Company, Ltd., Yokohama, 230-0045 Japan}
\author{Hitoshi Sumiya} 
\affiliation{Advanced Materials Laboratory, Sumitomo Electric Industries, Ltd., Itami, 664-0016 Japan}
\author{Takeshi Ohshima} 
\affiliation{Takasaki Advanced Radiation Research Institute, National Institutes for Quantum and Radiological Science and Technology, Takasaki, 370-1292, Japan }
\author{Junichi Isoya}
\affiliation{Faculty of Pure and Applied Sciences, University of Tsukuba, Tsukuba, 305-8573 Japan}
\author{J\"{o}rg Wrachtrup}
\affiliation{Institute of Physics, University of Stuttgart and Institute for Quantum Science and Technology IQST, 70174 Stuttgart, Germany}
\author{Arne Wickenbrock}
\affiliation{Johannes Gutenberg-Universit{\"a}t Mainz, 55128 Mainz, Germany}
\affiliation{Helmholtz Institut Mainz, 55099 Mainz, Germany}
\author{Dmitry Budker}
\affiliation{Johannes Gutenberg-Universit{\"a}t Mainz, 55128 Mainz, Germany}
\affiliation{Helmholtz Institut Mainz, 55099 Mainz, Germany}
\affiliation{Department of Physics, University of California, Berkeley, CA 94720-7300, USA}
\affiliation{Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
% \affiliation{$^{1}$Johannes Gutenberg-Universit{\"a}t  Mainz, 55128 Mainz, Germany \\  $^{2}$Helmholtz Institut Mainz, 55099 Mainz, Germany\\ $^{3}$Department of Physics, University of California, Berkeley, CA 94720-7300, USA\\ $^{4}$Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
 \date{\today}% It is always \today, today,
%              %  but any date may be explicitly specified

\end{comment}
% \section{Supplementary Information}
% \setcounter{figure}{0}
% \renewcommand{\thefigure}{S\arabic{figure}}
% \subsection{Illustration of the working principle of the transverse field detection.}
The PL-GSLAC feature changes its shape according to the applied transverse field, which, however, does not depend on the direction of the field in the $x$-$y$ plane. We approximate the PL-GSLAC feature as a function of transverse field by a 2D Lorentzian function symmetric around the $z$-axis, indicated in Fig.\,\ref{fig:xymethod} (a) (i). The maximum PL signal corresponds to zero transverse magnetic field and it decreases as the magnitude of the transverse field increases. When applying a transverse magnetic field rotating around the $z$-axis, the PL signal is reduced but remains constant (no oscillating component) in the absence of a transverse DC field, indicated by the red curve in Fig.\,\ref{fig:xymethod} (a) (ii). 
In the presence of a transverse field, the PL signal is off center from the coordinate origin and shows a minimum value when the rotating field reaches the same direction as the transverse field being interrogated, shown in Fig.\,\ref{fig:xymethod} (a) (iii), (iv) and (v). The difference between the PL signals with (red curve) and without (blue curve) applied transverse field is shown in Fig.\,\ref{fig:xymethod} (b). This is then demodulated by a LIA which delivers the information of both the amplitude and the angle of the magnetic field to be measured, as shown in Fig.\,\ref{fig:xymethod} (c).

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{fig6_xymethod.pdf}
\caption{(a) Simulated PL signals as a function of transverse field. The red curves are the trajectories of PL signals superimposed on the 2D Lorentzian contrast function. Figures i) to v), correspond to different show cases: i) no modulated fields and no bias fields, ii) with modulated fields but no bias fields (the time-averaged PL drops), iii) with modulated fields and bias field along $y$, iv) with modulated fields and bias field along $x$, v) with modulated fields and bias field in $x$-$y$ plane, respectively. (b) The simulated PL signals with modulating magnetic field in the presence/absence (red curve/blue curve) of a bias field. (c) Simulated PL signals [in the same coordinate system as in column (a)] as a function of the angle of the modulated field referenced to the -$x$-axis for transverse fields corresponding to (a) and (b).}
\label{fig:xymethod}
\end{figure*}
The $x$ and $y$ axes can be calibrated by tuning the reference phase of the modulation field. In our case, the measured $x$ and $y$ axes are set along the $x$- and $y$-modulating Helmholtz coils. The reference phase of the LIA was set so that a magnetic field along the $x$-axis corresponds to phase zero (and negative amplitude). The LIA output shows a maximum value at $0^o$ when applying a field along $x$-axis, shown in Fig.\,\ref{fig:xymethod} (c). An applied field in any other direction leads to an oscillating PL signal with a corresponding phase. Therefore, the phase output of the LIA is the angle between the transverse field to be measured and the defined $x$ and $y$ axes. 

The modulation field is generated by two Helmholtz coils driven by sinusoidally oscillating currents resulting in a transverse field amplitude of $\approx$20\,$\mu$T. The fields are oscillating at the same frequency but exhibit a relative phase shift of 90 degrees. The phase between these two modulating fields as well as the respective amplitudes are adjusted to via minimizing the magnitude output of the LIA without an applied transverse field. 
% \subsection{Demonstration of an $x$-$z$ measurement.}
% Full vector measurements of magnetic fields require a measurement in the $z$ direction. They are carried out by applying an additional modulated field along $z$ with a different frequency (than in the transverse direction) and demodulation of the PL signal. A matrix of 2D vector magnetic fields in $x$-$z$ plane was measured to demonstrate the method with various $B_x$ and $B_z$ in the range of $\pm3$ $\mu$T. The angle of the field can be calculated as $\arctan({B_z}/{B_x})$ from the applied currents and calibration factors of the two coils. Figure\,\ref{fig:xzdemonstration} shows that the ratios of the measured fields $B_z$ and $B_x$ correspond to different angles following the expected arctangent curve. The comparison corroborates the method's effectiveness.

% \begin{figure}
% \centering
% \includegraphics[width=\columnwidth]{fig5_zx_new.pdf}
% \caption{The ratios of measured fields $B_z/B_x$ corresponding to different angles are calculated from the applied fields in $x$-$z$ plane. The solid green line shows an arctangent dependence.}
% \label{fig:xzdemonstration}
% \end{figure}

%\end{document}

